Can't Touch This: Real-Time, Safe Motion Planning and Control for Manipulators Under Uncertainty

Ensuring safe, real-time motion planning in arbitrary environments requires a robotic manipulator to avoid collisions, obey joint limits, and account for uncertainties in the mass and inertia of objects and the robot itself. This paper proposes Autonomous Robust Manipulation via Optimization with Uncertainty-aware Reachability (ARMOUR), a provably-safe, receding-horizon trajectory planner and tracking controller framework for robotic manipulators to address these challenges. ARMOUR first constructs a robust controller that tracks desired trajectories with bounded error despite uncertain dynamics. ARMOUR then uses a novel recursive Newton-Euler method to compute all inputs required to track any trajectory within a continuum of desired trajectories. Finally, ARMOUR over-approximates the swept volume of the manipulator; this enables one to formulate an optimization problem that can be solved in real-time to synthesize provably-safe motions. This paper compares ARMOUR to state of the art methods on a set of challenging manipulation examples in simulation and demonstrates its ability to ensure safety on real hardware in the presence of model uncertainty without sacrificing performance. Project page: https://roahmlab.github.io/armour/.

==> algorithms/createTraj.tex <==
         %~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

\State{\bf parfor} $i \in N_T$ %// parallel for each time step

    \State\hspace{0.2in}{\bf for} $j = 1:n_q$ %// for each joint


        \State\hspace{0.4in}$\pz{\Zjt} \leftarrow \texttt{loadJRS}(\initdqj)$

        \State\hspace{0.4in}$\sigma \leftarrow (\initdqj - \avgkj)/(\delkj)$ %//


        \State\hspace{0.4in}$\pz{S_j(t)} \leftarrow \texttt{pzSlice}(\pz{\Zjt}, \sigma, s)$ 
    

        \State\hspace{0.4in}$\pz{R\jssmu} \leftarrow \texttt{pzRotMat}(\initqj)$
    
        
        % \State\hspace{0.4in}$\pz{\qi}, \pz{\qidot}, \pz{\qiddot}   \leftarrow \texttt{pzTraj}(\pz{S_i(t)})$
        \State\hspace{0.4in}$\pzqji, \pzqdji, \pzqddji   \leftarrow \texttt{pzTraj}(\pz{S_j(t)})$
        
        \State\hspace{0.4in}$\pz{\qi} \leftarrow \pz{R\jssmu} \odot \pz{\qi}$
        
        \State\hspace{0.4in}{\bf end for}
    
    \State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pzqji, \pzqdji, \pzqddji \,:\, j \in N_q,\ i \in N_T \} = \texttt{createTraj}(\initq,\initdq)$ \pat{this will change}}
\label{alg:create_traj}
\end{algorithm}


==> algorithms/deprecated/pzfk_deprecated.tex <==
         %~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

\State{\bf parfor} $t \in T$ %// parallel for each time step

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ %// for each joint
    \State\hspace{0.4in}$\pz{\pit} \leftarrow \pz{\mathbf{0}}$ %// initialize frame location 
        
    \State\hspace{0.4in}$\pz{\Rit} \leftarrow \pz{I_{3 \times 3}}$ %// initialize frame orientation
    
     \State\hspace{0.4in}{\bf for} $j = 1:i$
         \State\hspace{0.6in}$\lkvjt \leftarrow (\pz{\qjdot} - \avgkj)/(\delkj)$ 

        \State\hspace{0.6in}$\pz{\qj} \leftarrow \texttt{slice}(\pz{\qj}, \sym{\lkvjt}, \lkvjt)$ 
    
        \State\hspace{0.6in}$\pz{R\jssmu} \leftarrow \texttt{makeMatZono}(\pz{\qj})$ %// see
    
        \State\hspace{0.6in}$\pz{\pit} \leftarrow \pz{\pit} \oplus \pz{\Rit} \odot \pz{p_{j}^{j-1}}$
        
        \State\hspace{0.6in}$\pz{\Rit} \leftarrow \pz{\Rit} \odot  \pz{R\jssmu}$ 

    \State\hspace{0.4in}{\bf end for}
    
    \State\hspace{0.4in}$\pz{\FK_i(t)} \leftarrow \{ \pz{\Rit} ,  \pz{\pit} \}$ 
  
    
\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pz{\FK_i(t)}\,:\, i = 1,\cdots,n_q,\ t\in T\} = \texttt{PZFK}(\pz{\q},\pz{\qd})$}
\label{alg:compose_fk}
\end{algorithm}

==> algorithms/deprecated/pzfo2_deprecated.tex <==
%~~~~~~~~~~~~ Compose RS
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

% \State$\pz{q(0)}, \cdots, \pz{q(T)} \leftarrow \texttt{createTraj}(\hat{q}_0, \dot{\hat{q}}_0)$ 

\State{\bf parfor} $t \in T$ %// parallel for each time step

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ %// for each joint

    % \State\hspace{0.4in}$\sigma \leftarrow (\dot{\hat{q}}_{0,i} - \avgki)/(\delki)$ %// 

    % \State\hspace{0.4in}$\pz{\qi} \leftarrow \texttt{slice}(\pz{\Zit}, \sigma, s)$ 
    
    \State\hspace{0.4in}$\pz{R\issmu}, \pz{\nom{p\issmu}} \leftarrow \texttt{pzHomTrans}(\pz{\qi})$ 
    
    \State\hspace{0.4in}$\pz{\Vit} \leftarrow \pz{R\issmu}  \pz{L_i}$ %// init $\pz{\Vit}$ for link volume RS 
    
    \State\hspace{0.4in}$\pz{\Uit} \leftarrow \pz{\nom{p\issmu}}$ %// init rotatotope for joint location
    
    \State\hspace{0.4in}{\bf for} $j = (i-1):-1:1$  %// predecessor joints \jon{Fix R(t)}
    
        \State\hspace{0.6in}$\pz{\Vit} \leftarrow \pz{R\jssmu} \odot \pz{\Vit}$ %// rotate link volume 
        
        \State\hspace{0.6in}$\pz{\Uit} \leftarrow \pz{R\jssmu} \odot   \pz{\Uit}$ %// rotate joint location
    
    \State\hspace{0.4in}{\bf end for}

    \State\hspace{0.4in}{\bf for} $j = (i-1):-1:1$ %// predecessor joints

        \State\hspace{0.6in}$\pz{\Vit} \leftarrow \pz{\Vit} \oplus \pz{\Ujt}$ %// stack link on joints
        
    \State\hspace{0.4in}{\bf end for}
    
    \State\hspace{0.4in}$\pz{\FO_i(t)}  \leftarrow \pz{\Vit}$
    
    \State\hspace{0.2in}{\bf end for}
    
\State{\bf end parfor}

\end{algorithmic}

\caption{\small $\{\pz{\FO_i(t)}\,:\, i = 1,\cdots,n_q,\ t\in T\} = \texttt{PZFO}(\pz{q(0)}, \cdots, \pz{q(T)})$}
\label{alg:compose_fo}
\end{algorithm}



==> algorithms/deprecated/pzfo_deprecated.tex <==
%~~~~~~~~~~~~ Compose RS
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

\State{\bf parfor} $t \in T$ %// parallel for each time step

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ %// for each joint

    \State\hspace{0.4in}$\lkvit \leftarrow (\pz{\qidot} - \avgki)/(\delki)$ %// 

    \State\hspace{0.4in}$\pz{\qi} \leftarrow \texttt{slice}(\pz{\qi}, \sym{\lkvit}, \lkvit)$ 
    
    \State\hspace{0.4in}$\pz{R\issmu} \leftarrow \texttt{makeMatZono}(\pz{\qi})$ %// see
    
    \State\hspace{0.4in}$\pz{\Vit} \leftarrow \pz{R\issmu}  \pz{L_i}$ %// init $\pz{\Vit}$ for link volume RS 
    
    \State\hspace{0.4in}$\pz{\Uit} \leftarrow \pz{\nom{p\issmu}}$ %// init rotatotope for joint location
    
    \State\hspace{0.4in}{\bf for} $j = (i-1):-1:1$  %// predecessor joints \jon{Fix R(t)}
    
        \State\hspace{0.6in}$\pz{\Vit} \leftarrow \pz{R\jssmu} \odot \pz{\Vit}$ %// rotate link volume 
        
        \State\hspace{0.6in}$\pz{\Uit} \leftarrow \pz{R\jssmu} \odot   \pz{\Uit}$ %// rotate joint location
    
    \State\hspace{0.4in}{\bf end for}

    \State\hspace{0.4in}{\bf for} $j = (i-1):-1:1$ %// predecessor joints

        \State\hspace{0.6in}$\pz{\Vit} \leftarrow \pz{\Vit} \oplus \pz{\Ujt}$ %// stack link on joints
        
    \State\hspace{0.4in}{\bf end for}
    
    \State\hspace{0.4in}$\pz{\FO_i(t)}  \leftarrow \pz{\Vit}$
    
    \State\hspace{0.2in}{\bf end for}
    
\State{\bf end parfor}

\end{algorithmic}

\caption{\small $\{\pz{\FO_i(t)}\,:\, i = 1,\cdots,n_q,\ t\in T\} = \texttt{PZFO}(\pz{\q},\pz{\qd})$}
\label{alg:compose_fo}
\end{algorithm}

==> algorithms/deprecated/pzrnea_deprecated.tex <==
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
\State{\bf parfor} $t \in T$ %// parallel for each time step

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ %// for each joint
    \State\hspace{0.4in}$\lkvit \leftarrow (\pz{\qidot} - \avgki)/(\delki)$ %// 

    \State\hspace{0.4in}$\pz{\qi} \leftarrow \texttt{slice}(\pz{\qi}, \sym{\lkvit}, \lkvit)$ 
    % \State\hspace{0.4in}$\pz{\Zitv} \leftarrow \texttt{slice}(\pz{\Zit}, \sym{\lkvit}, \lkvit)$ %// slice JRS

    % \State\hspace{0.4in}$\pz{R_i(t)} \leftarrow \texttt{makeMatZono}(\pz{\Zit},\pz{\q})$ %// see
    
    \State\hspace{0.4in} $\pz{R\issmu} \gets \texttt{makeMatZono}(\pz{\qi})$ 
    
    \State\hspace{0.4in} $\pz{R\issm} \gets \texttt{transpose}(\pz{R\issmu})$
    
\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ %// for each joint (start of forward recursion)

    \State\hspace{0.4in} $\pz{\omega\iss} \gets \pz{R\issm} \bigodot \pz{\omega\issmm} \bigoplus \pz{\qidot}\zi$
    
    \State\hspace{0.4in} $\pz{\omega\issa} \gets \pz{R\issm} \bigodot \pz{\omega\issmma} \bigoplus \pz{\qaidot}\zi$
    
    \State\hspace{0.4in} $\pz{\dot{\omega}\iss} \gets \pz{R\issm} \bigodot \pz{\dot{\omega}\issmm} \bigoplus ((\pz{R\issm} \bigodot \pz{\dot{\omega}\issmm}) \bigotimes (\pz{\qidot} \zi)) \bigoplus \pz{\qiddot}\zi$
    
    \State\hspace{0.4in} $\pz{a\iss} \gets (\pz{R\issm} \bigodot \pz{a\issmm}) \bigoplus (\pz{\dot{\omega}\iss} \bigotimes \pz{p\issmi}) \bigoplus (\pz{\omega\iss} \bigotimes (\pz{\omega\issa} \times \pz{p\issmi}))$
    
    \State\hspace{0.4in} $\pz{a\issc} \gets \pz{a\iss} \bigoplus (\pz{\dot{\omega}\iss} \bigotimes \pz{c\iss}) \bigoplus (\pz{\omega\iss} \bigotimes (\pz{\omega\issa} \bigotimes \pz{c\iss})) $
    
    \State\hspace{0.4in} $\pz{F\iss} \gets \pz{m_i} \bigodot \pz{a\issc}$
    
    \State\hspace{0.4in} $\pz{N\iss} \gets \pz{I\iss} \bigodot \pz{\dot{\omega}\iss} \bigoplus (\pz{\omega\issa}  \bigotimes (\pz{I\iss} \bigodot \pz{\omega\iss})) $

\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}Initialize $\pz{f^{n_q+1}_{n_q+1}}, \pz{n^{n_q+1}_{n_q+1}}, \pz{R^{n_q}_{n_q+1}}$

\State\hspace{0.2in}{\bf for} $i = n_q:-1:1$ %// for each joint (start of backward recursion)

\State\hspace{0.4in} $\pz{f\iss} \gets (\pz{R\issp} \bigodot \pz{f^{i+1}_{i+1}}) \bigoplus \pz{F\iss} $

\State\hspace{0.4in} $\pz{n\iss} \gets (\pz{R\issp} \bigodot \pz{n^{i+1}_{i+1}}) \bigoplus (\pz{c\iss} \bigotimes \pz{F\iss}) \bigoplus (\pz{p\issmi} \bigotimes (\pz{R\issp} \bigodot \pz{f^{i+1}_{i+1}})) \bigoplus \pz{N\iss} $ 
\State\hspace{0.4in} $\pz{\uit} \gets \pz{n\iss} \bigodot z_i$

\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}
\end{algorithmic}
\caption{\small $\{\pz{\uit}\,:\, i = 1,\cdots,n_q,\ t\in T\} = \texttt{PZRNEA}(\pz{\q},\pz{\qd}, \pz{\qadot}, \pz{\qdd}, \pz{\Delta})$}
\label{alg:PZRNEA}
\end{algorithm}

==> algorithms/iirnea.tex <==
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
\State{\bf parfor} $t \in T$ // parallel for each time step

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ // for each joint

    
    \State\hspace{0.4in} $\iv{R\issmu} \gets \texttt{makeMatZono}(\iv{\qi})$ 
    
    \State\hspace{0.4in} $\iv{R\issm} \gets \texttt{transpose}(\iv{R\issmu})$
    
\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}{\bf for} $i = 1:n_q$ // for each joint (start of forward recursion)

    \State\hspace{0.4in} $\iv{\omega\iss} \gets \iv{R\issm} \bigodot \iv{\omega\issmm} \bigoplus \iv{\qidot}\zi$
    
    \State\hspace{0.4in} $\iv{\omega\issa} \gets \iv{R\issm} \bigodot \iv{\omega\issmma} \bigoplus \iv{\qaidot}\zi$
    
    \State\hspace{0.4in} $\iv{\dot{\omega}\iss} \gets \iv{R\issm} \bigodot \iv{\dot{\omega}\issmm} \bigoplus ((\iv{R\issm} \bigodot \iv{\dot{\omega}\issmm}) \bigotimes (\iv{\qidot} \zi)) \bigoplus \iv{\qiddot}\zi$
    
    \State\hspace{0.4in} $\iv{a\iss} \gets (\iv{R\issm} \bigodot \iv{a\issmm}) \bigoplus (\iv{\dot{\omega}\iss} \bigotimes \iv{p\issmi}) \bigoplus (\iv{\omega\iss} \bigotimes (\iv{\omega\issa} \times \iv{p\issmi}))$
    
    \State\hspace{0.4in} $\iv{a\issc} \gets \iv{a\iss} \bigoplus (\iv{\dot{\omega}\iss} \bigotimes \iv{c\iss}) \bigoplus (\iv{\omega\iss} \bigotimes (\iv{\omega\issa} \bigotimes \iv{c\iss})) $
    
    \State\hspace{0.4in} $\iv{F\iss} \gets \iv{m_i} \bigodot \iv{a\issc}$
    
    \State\hspace{0.4in} $\iv{N\iss} \gets \iv{I\iss} \bigodot \iv{\dot{\omega}\iss} \bigoplus (\iv{\omega\issa}  \bigotimes (\iv{I\iss} \bigodot \iv{\omega\iss})) $

\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}Initialize $\iv{f^{n_q+1}_{n_q+1}}, \iv{n^{n_q+1}_{n_q+1}}, \iv{R^{n_q}_{n_q+1}}$

\State\hspace{0.2in}{\bf for} $i = n_q:-1:1$ // for each joint (start of backward recursion)

\State\hspace{0.4in} $\iv{f\iss} \gets (\iv{R\issp} \bigodot \iv{f^{i+1}_{i+1}}) \bigoplus \iv{F\iss} $

\State\hspace{0.4in} $\iv{n\iss} \gets (\iv{R\issp} \bigodot \iv{n^{i+1}_{i+1}}) \bigoplus (\iv{c\iss} \bigotimes \iv{F\iss}) \bigoplus (\iv{p\issmi} \bigotimes (\iv{R\issp} \bigodot \iv{f^{i+1}_{i+1}})) \bigoplus \iv{N\iss} $ 
\State\hspace{0.4in} $\iv{\uit} \gets \iv{n\iss} \bigodot z_i$

\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}
\end{algorithmic}
\caption{\small $\{\iv{\uit}\,:\, j \in N_q,\ t\in T\} = \texttt{PZRNEA}(\iv{\q},\iv{\qd}, \iv{\qadot}, \iv{\qdd}, \iv{\Delta})$ \jon{fix long lines, double check $p_i^{i-1}$}}
\label{alg:PZRNEA}
\end{algorithm}

==> algorithms/pzfo.tex <==
         %~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
 \jon{define pzHomTrans}
\begin{algorithmic}[1]


\State{\bf parfor} $i = 1:\nt$ %// parallel for each time step

\State\hspace{0.2in}{\bf for} $j = 1:\nq$ %// for each joint
    \State\hspace{0.4in}$\pz{p_j}(\pzqi) \leftarrow \pz{\mathbf{0}}$ %// initialize frame location 
        
    \State\hspace{0.4in}$ \pz{R_j}(\pzqi) \leftarrow \pz{I_{3 \times 3}}$ %// initialize frame orientation
    
     \State\hspace{0.4in}{\bf for} $l = 1:j$

        \State\hspace{0.6in}$\pz{R_{l}^{l-1}}(\pzqli), \pz{\nom{p\lssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
        \State\hspace{0.6in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)  \odot \pz{p_{l}^{l-1}}$
        
        \State\hspace{0.6in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_j}(\pzqi) \odot  \pz{R_{l}^{l-1}}(\pzqli)$ 

    \State\hspace{0.4in}{\bf end for}
    

     \State\hspace{0.4in}$\pz{\FO_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus  \pz{R_j}(\pzqi) \odot \pz{L_j}$ 
  
    
\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pz{\FO_j}(\pzqi)\,:\, j \in \Nq,\ i \in \Nt \} = \texttt{PZFO}(\{ \pzi{q_j} \,:\, j \in \Nq,\ i \in \Nt \})$}
\label{alg:compose_fo}
\end{algorithm}

==> algorithms/rnea.tex <==
\begin{algorithm}[t]
\jon{define makeHomTrans, double check $p_j^{j-1}$} 
\small
\begin{algorithmic}[1]
\State Compute $\dot{q}_a$ and $\ddot{q}_a$ using \eqref{eq:modified_ref}.
\State Initialize base linear acceleration $a_0^0$.
\State{\bf parfor} $t \in T$ // parallel for each time step

\State\hspace{0.2in}{\bf for} $j = 1:\nq$ // for each joint
    
    \State\hspace{0.4in} $\nom{R\jssmu}, p\jssmu \gets \texttt{TransMat}(\nom{\qj})$ \Ram{this operation has not been defined}\jon{Eq 38}
    
    \State\hspace{0.4in} $\nom{R\jssm} \gets \texttt{transpose}(\nom{R\jssmu})$
    
\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}{\bf for} $j = 1:\nq$ // for each joint (forward recursion)

    \State\hspace{0.4in} $\nom{\omega\jss} \gets \nom{R\jssm} \bigodot \nom{\omega\jssmm} \bigoplus \nom{\qdj}\zi$  \Ram{what does $\zi$ mean?}
    
    \State\hspace{0.4in} $\nom{\omega\jssa} \gets \nom{R\jssm} \bigodot \nom{\omega\jssmma} \bigoplus \nom{\qajdot}\zi$
    
    \State\hspace{0.4in} $\nom{\dot{\omega}\jss} \gets \nom{R\jssm} \bigodot \nom{\dot{\omega}\jssmm} \bigoplus \newline \hspace*{7em} \bigoplus ((\nom{R\jssm} \bigodot \nom{\omega\jssmma}) \bigotimes (\nom{\qdj} \zi)) \bigoplus \nom{\ddot{q}_{a,j}(t)}\zi $
    
    \State\hspace{0.4in} $\nom{a\jss} \gets (\nom{R\jssm} \bigodot \nom{a\jssmm}) \bigoplus (\nom{\dot{\omega}\jss} \bigotimes \nom{p\jssmj}) \bigoplus \newline \hspace*{7em} \bigoplus (\nom{\omega\jss} \bigotimes (\nom{\omega\jssa} \times \nom{p\jssmj}))$
    
    \State\hspace{0.4in} $\nom{a\jssc} \gets \nom{a\jss} \bigoplus (\nom{\dot{\omega}\jss} \bigotimes \nom{c\jss}) \bigoplus (\nom{\omega\jss} \bigotimes (\nom{\omega\jssa} \bigotimes \nom{c\jss})) $
    
    \State\hspace{0.4in} $\nom{F\jss} \gets \nom{m_i} \bigodot \nom{a\jssc}$
    
    \State\hspace{0.4in} $\nom{N\jss} \gets \nom{I\jss} \bigodot \nom{\dot{\omega}\jss} \bigoplus (\nom{\omega\jssa}  \bigotimes (\nom{I\jss} \bigodot \nom{\omega\jss})) $

\State\hspace{0.2in}{\bf end for}

\State\hspace{0.2in}Initialize $\nom{f^{\nq+1}_{\nq+1}}, \nom{n^{\nq+1}_{\nq+1}}, \nom{R^{\nq}_{\nq+1}}$ \jon{explains how this is initialized}

\State\hspace{0.2in}{\bf for} $j = \nq:-1:1$ // for each joint (backward recursion)

\State\hspace{0.4in} $\nom{f\jss} \gets (\nom{R\jssp} \bigodot \nom{f^{j+1}_{j+1}}) \bigoplus \nom{F\jss} $

\State\hspace{0.4in} $\nom{n\jss} \gets (\nom{R\jssp} \bigodot \nom{n^{j+1}_{j+1}}) \bigoplus (\nom{c\jss} \bigotimes \nom{F\jss}) \bigoplus \newline \hspace*{7em} \bigoplus (\nom{p\jssmj} \bigotimes (\nom{R\jssp} \bigodot \nom{f^{j+1}_{j+1}})) \bigoplus \nom{N\jss} $ 
\State\hspace{0.4in} $\nom{\ujt} \gets z_j^\top \nom{n\jss} $

\State\hspace{0.2in}{\bf end for}

\State{\bf end parfor}
\end{algorithmic}
\caption{\small $\{\ujt\,:\, j \in \Nq,\ t\in T\} = \texttt{RNEA}(\qA(t), \nom{\Delta}, a_0^0)$
\shrey{Do we really need both algs. 1 and 2?}
\pat{add gravity term}
\fix{done}
}
\label{alg:RNEA}
\end{algorithm}

==> algorithms/slice.tex <==
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
    \State // Let $Z = (x,g^i,\sym{\beta^i})^p$ denote the input zonotope or rotatotope

    \State  $Z_{\regtext{sliced}} \leftarrow (x,g^i,\sym{\beta^i})^p$ // allocate output

    \State{\bf for} $i = 1,\cdots,p$ // iterate over generator/indeterminate pairs
    
    \State\hspace{0.2in}{\bf for} $j = 1,\cdots,n$  // iterate over input values
    
    \State\hspace{0.4in}{\bf if} $\sym{\sigma^j} \in \sym{\beta^i}$
    
    \State\hspace{0.6in} $g^i \leftarrow \sigma^j g^i$ // multiply generator by value
    
    \State\hspace{0.6in} $\sym{\beta^i} \leftarrow \sym{\beta^i} \setminus \sym{\sigma^j}$ // remove evaluated indeterminate

    \State\hspace{0.4in}{\bf end if}
    
    \State\hspace{0.2in}{\bf end for}
    
    \State\hspace{0.2in}{\bf if} $\sym{\beta^i} = \emptyset$ // if fully-sliced, then $g^i$ is no longer needed
    
    \State\hspace{0.4in} $x \leftarrow x + g^i$ and $g^i \leftarrow \emptyset$ // shift center, remove generator
    
    % \State\hspace{0.4in} $g^i \leftarrow \emptyset$ // generator is no longer needed 
    
    \State\hspace{0.2in}{\bf end if}
    
    \State{\bf end for}
    
    \end{algorithmic}
\caption{\small $Z_{\regtext{sliced}} = \slice\left(Z, \{\sym{\sigma^j}\}_{j=1}^n, \{\sigma^j\}_{j=1}^n\right)$}
\label{alg:slice}
\end{algorithm}

==> sections/00_outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]
\1 Introduction
    \2 Background + Motivation
    \2 Related Work \shrey{I moved this to its own section}
        
    \2 Contributions and Overview of Proposed Method
        \3 Incorporate dynamics into ARMTD \cite{holmes2020armtd}
        \3 Extend interval RNEA to incorporate parameterized trajectories
        \3 Demonstrate robust pick-and-place in clutter
        
    \2 Paper Organization
    
\1 Related Work

\1 Controller Design
    \2 Jon fill this in?
    \2 Theoretical Overview
    \2 Numerical Implementation
    
\1 Trajectory Design

\1 Planning Formulation
    \2 Overview of timing
    \2 Optimization problem
    
\1 Planning Algorithm Theory
    \2 Time partition
    \2 Trajectory overapproximation
    \2 Reachable sets
        \3 Forward kinematics/occupancy
        \3 Nominal + robust input
    \2 PZ optimization problem
    
\1 Planning Algorithm Implementation
    \2 Offline trajectory reachable sets
    \2 FK, FO, RNEA algorithm implementation
        \3 details... reduce PZs after any operation
    \2 Constraint implementation
        \3 Mostly "box" constraints with PZ
        \3 Collision-avoidance as polytopes
        \3 details... make all "non-fully-k-sliceable" terms independent
    \2 Optimization problem implementation
    \2 Getting analytical gradients
        
        

% \1 Offline Reachability Analysis
%     \2 Decide on OZ or PZ
%     \2 Theoretical Overview
%     \2 Numerical Implementation

% \1 Online Trajectory Planning
%     \2 Theoretical Overview
%     \2 Numerical Implementation

\1 Simulation Results

\1 Hardware Results

\1 Conclusion
\end{outline}

==> sections/07_implementation.tex <==
\section{\methodname{} Implementation}
\label{sec:implementation}

This section describes our implementation of the planning algorithm formulated in Section \ref{sec:algorithm_theory} and how to apply it while performing real-time control in dynamically feasible fashion while avoiding obstacles and satisfying input constraints. 
To simplify exposition in Section \ref{subsec:implementation_trajectories}, we begin by proposing an example desired trajectory that satisfies Definition \ref{def:traj_param} and describe how to construct a polynomial zonotope overapproximation to it as was described in Section \ref{subsec:pz_traj_rep}.
Next in Section \ref{subsec:implementation_constraints}, we describe how to use this polynomial zonotope representation to write down constraints \eqref{eq:pz_optpos}-\eqref{eq:pz_optposcon}. 
Finally in Section \ref{subsec:implementation_online}, we summarize the online operation of \methodname{}.

\subsection{An Example Desired Trajectory}
\label{subsec:implementation_trajectories}
% \input{algorithms/createTraj}

This work uses degree 5 Bernstein polynomials to parameterize the desired trajectories of the arm.
Letting $T = [0, 1]$, the Bernstein polynomials take the form
\begin{equation}
    \label{eq:q_bernstein_polynomial}
    \qdeskj = \sum_{l= 0}^{5} \beta_{j, l}(k) b_{j, l}(t),
\end{equation}
where $\beta_{j, l}(k) \in \R$ are the Bernstein Coefficients and $b_{j, l}: T \to \R$ are the Bernstein Basis Polynomials of degree 5 given by
\begin{equation}
    \label{eq:bernstein_basis_polynomial}
    b_{j, l}(t) = {5\choose l}t^{l}(1 - t)^{5 -l},
\end{equation}
for each $l \in \{0, \ldots, 5\}$.
Notice from Definition \ref{def:traj_param} that the first and second properties of trajectory parameters constrain the initial position, velocity, and acceleration of the trajectory to match the initial condition, and require the final velocity and acceleration to be $0$.
These properties fix five of the six Bernstein coefficients $\beta_{j, \nu}$ as
\begin{align}
    \label{eq:bernstein_coeff}
    \beta_{j, 0}(k) &= \initqj \\
    \beta_{j, 1}(k) &= \tfrac{1}{5}(\initdqj + 5\beta_{j, 0}) \\
    \beta_{j, 2}(k) &= \tfrac{1}{20}(\initddqj + 40\beta_{j, 1} - 20\beta_{j, 0})\\
    \beta_{j, 3}(k) &= \tfrac{1}{20}(0 + 40\beta_{j, 4} - 20\beta_{j, 5})\\
    \beta_{j, 4}(k) &= \tfrac{1}{5}(0 + 5\beta_{j, 5}).
\end{align}
Note because the first five Bernstein coefficients are fixed, they are not a function of the trajectory parameter, so we drop the dependence on $k$ for these coefficients.
We let the last coefficient $\beta_{j, 5}$ be
\begin{equation}
    \label{eq:bernstein_k_coeff}
    \beta_{j, 5}(k) = \kjscale \kj + \kjoffset
\end{equation}
where $\kjscale$ and $\kjoffset \in \R$ are user-specified constants.
The coefficient $\beta_{j, 5}$ equals the final position $q_j(1; k)$ at time $t = 1$, so the choice of trajectory parameter $k_j$ determines this value.
% Note that with this formulation, $\beta_{j, 3} = \beta_{j, 4} = \beta_{j, 5}$.

% Similarly, we may write the interval $\Kj = \iv{-1, 1}$ as a polynomial zonotope $\pz{\Kj} = k_j$ with $k_j \in \iv{-1, 1}$.
We construct the polynomial zonotope representation $\pzqdesji$ by plugging in $\pz{T_i}$ from \eqref{eq:time_pz} and $\pz{\Kj}$.
Letting $\pzgreek{\beta}_\pz{j, 5}(\pz{K}) = \kjscale \pz{\Kj} + \kjoffset$, and plugging $\pz{T_i}$ into the basis polynomials \eqref{eq:bernstein_basis_polynomial}, we obtain
\begin{equation}
    \pzqdesji = \left( \sum_{l = 0}^{4} \beta_{j, l} \pz{b_{j, l}}(\pz{T_i}) \right) \oplus \bm{\beta}_\mathbf{j, 5}(\pz{K})\pz{b_{j, 5}}(\pz{T_i}),
\end{equation}
The desired velocity and acceleration polynomial zonotopes $\pzqddesji$ and $\pzqdddesji$ can be similarly computed.
These desired trajectory polynomial zonotopes are combined with the tracking error polynomial zonotopes to get $\pzqi$ and $\pzqdi$ as in \eqref{eq:pz_pos} and \eqref{eq:pz_vel}, as well as $\pzqdai$ and $\pzqddai$ as in \eqref{eq:pz_mod_traj}.
To summarize, by specifying the initial condition of the desired trajectory, \emph{i.e.}, $(\initq, \initdq, \initddq)$, one can construct the polynomial zonotope representation of the desired trajectory and all of its variants.
% Recalling $\pz{\Kj}$ from Definition \ref{def:pz_Kj} and plugging these into \eqref{eq:traj_acc_parameterization}--\eqref{eq:traj_pos_parameterization} we obtain

% \pat{can make this shorter by just writing velocities in terms of $\qdeskjddot$ and positions in terms of $\qdeskjdot$}
% \begin{align}
%     \pzqdddesji &= \begin{cases}
%         \kjscale \pz{\Kj}, &t \in [0,t\plan) \\
%         \pz{\ddot{q}_{j, \regtext{brake}}} &t \in [t\plan,\tfin]
%     \end{cases}, \\
%     \pzqddesji &= \begin{cases}
%         \initdqj + \kjscale \pz{\Kj} \pzi{T}, &i \in [1, \frac{t\plan}{\timestep}) \\
%         \pz{\dot{q}_{j, \plan}} + \pz{\ddot{q}_{j, \regtext{brake}}}(\pzi{T} - t\plan), &i \in [\frac{t\plan}{\timestep}, \nt ],
%     \end{cases}, \\
% % \end{equation}
% % \begin{equation}
% %     \qdeskj \in \initqj + \initdqj \iv{0, \timestep} + \frac{1}{2}k_j \iv{0, \timestep}^2.
% % \end{equation}
% % This set can be represented as a polynomial zonotope.
% % Letting $\pz{t} = \frac{1}{2}\timestep + \frac{1}{2} \timestep \beta$, and $\pz{k_j} = \avgkj + \delkj \lambda$, then \begin{equation}
%     % \pzqdesji \coloneqq \initqj + \initdqj \pzi{t} + \frac{1}{2} \pz{K_j} \odot \pzi{t}^2.
%     \pzqdesji &= \begin{cases}
%         \initqj + \initdqj \pzi{t} +  \frac{1}{2}\kjscale \pz{\Kj} \pzi{T}^2, &i \in [0, \frac{t\plan}{\timestep} - 1) \\
%         \pz{q_{j, \plan}} + \pz{\dot{q}_{j, \plan}}(\pzi{T} - t\plan) + \frac{1}{2}\pz{\ddot{q}_{j,\regtext{brake}}}(\pzi{T} - t\plan)^2 &i \in [\frac{t\plan}{\timestep} - 1, \frac{\tfin}{\timestep} - 1].
%     \end{cases},
% \end{align}
% where $\pz{\dot{q}_{j, \plan}} = \initdqj + \kjscale \pz{K_j} t\plan$, $\pz{\ddot{q}_{j, \regtext{brake}}} = \frac{-\pz{\dot{q}_{j, \plan}}}{\tfin - t\plan}$, and $\pz{q_{j, \plan}} = \initqj + \initdqj t\plan +  \frac{1}{2}\kjscale \pz{\Kj} t\plan^2$.



\subsection{Constraints}\label{subsec:implementation_constraints}

We now implement joint limits, collision avoidance, and input constraints.
Recall that $\setop{sup}$ and $\setop{inf}$ overapproximate the bounds of a polynomial zonotope explicitly as in \eqref{eq:pz_sup} and \eqref{eq:pz_inf}, meaning that we do not need to optimize over the elements of a PZ to compute any of the following constraints.

% \subsection{Position and Orientation Constraints}
\subsubsection{Joint Limit Constraints}
\label{subsec:implementation_joint_constraints}
We generate constraints that ensure that the subsets of possible joint positions $\pzqki$ and joint velocities $\pzqdki$ for a given $k \in \pz{K}$ are within the allowable joint limits.
We let
\begin{align}
    h_{q^-}(i, j, k) &= -(\setop{inf}(\pzqjki) - \qlim^-) \\
    h_{q^+}(i, j, k) &= -(\qlim^+ - \setop{sup}(\pzqjki))
\end{align}
where $h_{q^-}(i, j, k) \leq 0$ and $h_{q^+}(i, j, k) \leq 0$ ensure that the joint position limits are satisfied.
Similarly, let
\begin{align}
    h_{\dot{q}^-}(i, j, k) &= -(\setop{inf}(\pzqdjki) - \dqlim^-) \\
    h_{\dot{q}^+}(i, j, k) &= -(\dqlim^+ - \setop{sup}(\pzqdjki))
\end{align}
where $h_{\dot{q}^-}(i, j, k) \leq 0$ and $h_{\dot{q}^+}(i, j, k) \leq 0$ ensure the joint velocity limits are satisfied.

% \input{algorithms/pzfk}
\subsubsection{Collision Avoidance Constraints}
\label{subsec:implementation_collision_constraints}
% \label{sec:collision_avoidance_implementation}
% The Polynomial Zonotope Forward Kinematics Algorithm (PZFK), detailed in Algorithm \ref{alg:compose_fk}, is used to compute sets of positions and orientations of each joint from the set of possible configurations $\pzqi$.
% Next, the Polynomial Zonotope Forward Occupancy Algorithm (PZFO), detailed in Algorithm \ref{alg:compose_fo}, is identical to the PZFK algorithm but is applied to the volume of each link rather than joint positions.
% \shrey{Do these need to be different algorithms?
% Maybe it would be sufficient to put an if statement in Algorithm 4.}
The forward occupancy PZ $\pzFOjKi$ produced by \eqref{eq:pz_forward_occupancy_j} overapproximates all reachable positions of points on the $j$\ts{th} link for the $i$\ts{th} time subinterval.
% Crucially, $\pzi{\FO_j(\pzqi)}$ depends on our choice of trajectory parameter $k$.
Our goal is to generate constraints which ensure that the subset of $\pzFOjKi$ for a particular $k$ do not intersect with any obstacles $O \in \obsset$.
% The subset of $\pzFOjKi$ corresponding to a particular $k$ is given by $\pzFOjki$.
These constraints are similar to those in \cite[Section 4]{holmes2020armtd}, but are updated to use the more general polynomial zonotope set representation.

Because the obstacles are convex polytopes (Assum. \ref{assum:obstacles}), one can compute a halfspace representation of obstacle $O$ given by $\Aobs \in \R^{\nf \times 3}$ and $\bobs \in \R^{\nf}$, where $\nf$ is the number of faces of $O$.
A point $p_1 \in \R^{3}$ is contained within the obstacle if and only if $\Aobs p_1 - \bobs \leq 0$, where the inequality is taken element-wise.
Therefore, $p_1$ lies outside the obstacle if any of the inequalities do not hold.
More succinctly, $p_1 \not \in O \iff \max(\Aobs p_1 - \bobs) > 0$, where the max is taken element-wise.
This implies that $\pzFOjki \cap O = \emptyset \iff \max(\Aobs p_1 - \bobs) > 0, \; \forall p_1 \in \pzFOjki$.
The expression $\Aobs\pzFOjki - \bobs$ yields an $\nf \times 1$ polynomial zonotope.
The constraint that $\pzFOjki$ does not intersect $O$ can be written as $\hobs(i, j, k, O) < 0$, where 
\begin{equation}
    \hobs(i, j, k, O) = -\max{(\setop{inf}(\Aobs\pzFOjki - \bobs))}
\end{equation}
and the $\max$ is taken element-wise.
% \pat{... do we need to explain how to take this max? basically there's $\nf$ $1$-dimensional PZs, and $k$ has been sliced out, so we can treat each as an interval. Then we take the supremum of each interval.}
% Though $\texttt{slice}(\pzi{\FO_j}, \kvar, k)$ is itself a polynomial zonotope, we can overapproximate it using a zonotope as in Lemma \ref{lem:zono_over_pz}.
% Note that by Assum. \ref{assum:obstacles}, each $O \in \obsset$ is represented by a zonotope.
% Therefore, we can enforce $\texttt{slice}(\pzi{\FO_j}, k, \cdot) \cap O = \emptyset \quad \forall O \in \obsset$ by ensuring two zonotopes do not intersect.

% % \pat{copied and pasted:}
% \begin{lem}\label{lem:zono_int}
% \cite[Lemma 5.1]{guibas2003zonotopes}
% % For two zonotopes $X = (x, g^i, \sym{\bt^i})^n$ and $Y = (y, g^j, \sym{\bt^j})^m$, $X \cap Y \neq \emptyset$ iff $y$ is in the zonotope $X\buf = (x, g^i, \sym{\bt^i})^n \oplus (0, g^j, \sym{\bt^j})^m$, where the subscript indicates $X$ is buffered by the generators of $Y$.
% Given zonotopes $Z_1$ and $Z_2$ (with centers $c_1$ and $c_2$ respectively), $Z_1 \cap Z_2 \not = \emptyset \iff c_2 \in Z_{1, \buf} = Z_1 \oplus (Z_2 - c_2)$.
% % , where the subscript indicates $A$ is buffered by the generators of $B$.
% % \begin{rem}\label{rem:halfspace_repr}
% \end{lem}

% \noindent In other words, checking if $Z_1$ and $Z_2$ intersect is equivalent to checking if $c_2$ is in a buffered version of $Z_1$ that has had the generators of $Z_2$ added to it.
% Since zonotopes are convex polytopes \cite{guibas2003zonotopes}, by \cite[Theorem 2.1]{althoff2010reachability}, one can implement Lemma \ref{lem:zono_int} by computing a \defemph{half-space representation} $(A\buf,b\buf)$ of $Z_{1,\buf}$ for which $A\buf c_2 - b\buf \leq 0 \iff c_2 \in X\buf$, where the inequality is taken elementwise.
% Using this representation, $Z_1 \bigcap Z_2 = \emptyset \iff \max(A\buf c_2 - b\buf) > 0$.
% We can use Lemma \ref{lem:zono_int} for collision avoidance by replacing $Z_1$ (resp. $Z_2$) with a zonotope representing the arm (resp. an obstacle).
% \input{algorithms/pzfo}

\subsubsection{Input Constraints}
\label{subsec:implementation_input_constraints}
% As written in \eqref{eq:pz_nominal_input}, the computation of the nominal input $\bm{\tau}(\pzqAi,\Delta_0)$ requires finding the mass matrix and Coriolis and gravitational terms.
% Instead, a more direct approach is to use a modified Recursive Newton-Euler Algorithm (RNEA) to compute $\bm{\tau}(\pzqAi,\Delta_0)$, which circumvents the computation of these terms.
% Here, we introduce the Polynomial Zonotope RNEA (PZRNEA), detailed in Algorithm \ref{alg:PZRNEA}.
% Note just as in the original RNEA and IRNEA Algorithms, we have suppressed the dependence on $\pzi{q_j}$ in $\pz{R_{j-1}^{j}}$.
% PZRNEA takes as inputs $\pzqAi$, and the nominal inertial parameters $\nomparams$ to find the nominal input:
% % \Ram{should this be PZ-ed?} \pat{I think we can go either way... The nominal params are just a vector, so converting that to a pz is trivial. For the interval params, I added \eqref{eq:int_to_pz} to show how to turn an interval to a PZ... so the conversions are there implicitly but idk if we should make it explicit} 
% % Here we use polynomial zonotopes and a modified RNEA algorithm, called Polynomial Zonotope RNEA (PZRNEA), to construct input constraints that are satisfied over the entire duration of a parameterized trajectory.
% \begin{align}
%   \bm{\tau}(\pzqAi,\Delta_0)= \texttt{PZRNEA}(\pzqAi, \nomparams).
% %   &+ \pzi{-\robcoeff \frac{\robr}{\norm{\robr}}} \\
% %   &\jon{\text{how to express robust input?}} \\
% \end{align}
% \input{algorithms/pzrnea}

% Note from \eqref{eq:pz_robust_input_bound}, creating $\pzi{v}$ requires polynomial zonotopes representing possible CBF values $\pzi{h}$ as well as possible disturbances $\pzi{w}$.
% To obtain $\pzi{w}$, we first get $\bm{\tau}_\mathbf{int}$ using the interval inertial parameters $\intparams$ \Ram{should this be $\bm{\Delta}$?}:
% \begin{equation}
    % \bm{\tau}_\mathbf{int} = \texttt{PZRNEA}(\pzqi, \pzqdi, \pzqdai, \pzqddai, \intparams).
% \end{equation}
% Then, $\pzi{w} = \pzi{\tau_\regtext{int}} - \pzi{\tau}$ as in \eqref{eq:pz_disturbance}.

% We use PZRNEA to compute $\pzi{h}$ by altering the inputs to the algorithm.
% Let
% \pat{remove this???}
% \begin{equation}
%     \pzi{V} = \frac{1}{2}\pzi{r}^\top \left( \pz{M}(\pzqi, \intparams) \pzi{r} \right),
% \end{equation}
% where the term 
% \begin{equation}
%     \pz{M}(\pzi{q}, \intparams) \pzi{r} = \texttt{PZRNEA}(\pzqi, \pz{0}, \pz{0}, \pzi{r}, \intparams).
% \end{equation}
% \pat{and the RNEA is used with gravity set to zero...}
% Then, we may obtain $\pzi{h}$ as
% \begin{equation}
%     \pzi{h} = -\pzi{V} + \roblevel
% \end{equation}
% as in \eqref{eq:CBF_defn}.

% Using $\pzi{w}$ and $\pzi{h}$ and plugging into

The nominal input polynomial zonotope $\bm{\tau}(\pzqAi,\Delta_0)$ is computed using PZRNEA as in \eqref{eq:pz_nominal_pzrnea}.
As discussed in Lemma \ref{thm:robust_input_bound}, we use PZRNEA to assist in constructing the robust input bound that generates $\pz{ v }(\pzqAi,\Delta_0,[\Delta])$ \eqref{eq:pz_robust_input} as well.
First, we construct $\pz{w}(\pzi{\qA},\nomparams,\intparams)$ using PZRNEA as in \eqref{eq:pz_disturbance}.
Plugging $\pz{w}(\pzi{\qA},\nomparams,\intparams)$, the uniform bound \eqref{eq:ultimate_bound_defn}, the eigenvalue bounds from Assumption \ref{ass:eigenvalue_bound}, and the form of $\alpha$ as in \eqref{eq:alpha_linear} into
\eqref{eq:pz_robust_coeff}, we may construct $\pz{ v }(\pzqAi,\Delta_0,[\Delta])$ as in \eqref{eq:pz_robust_input}.
Finally, combining $\bm{\tau}(\pzqAi,\Delta_0)$ and $\pz{ v }(\pzqAi,\Delta_0,[\Delta])$ yields $\pzujki$ as in \eqref{eq:pz_input}, which is then used to construct input constraints for a polynomial optimization problem.
In particular, we let
\begin{align}
    h_{u^-}(i, j, k) &= -(\setop{inf}(\pzki{u_j}) - \ulim^-) \\
    h_{u^+}(i, j, k) &= -(\ulim^+ - \setop{sup}(\pzki{u_j}))
\end{align}
where $h_{u^-}(i, j, k) < 0$ and $h_{u^-}(i, j, k) < 0$ ensures the input limits are satisfied.

% \subsection{A Note on Constraint Formulation}
% Most of the constraints found within the optimization problem involve ensuring a polynomial zonotope is contained within an interval.
% In practice, we enforce this constraint using two constraints, which we explain presently.
% Consider a polynomial zonotope $\pzi{P}$, which we slice by $k \in K$, yielding $\pzki{P}$.
% Say we want $\pzki{P}$ to be contained in the interval $\iv{a, b}$, i.e. $\pzki{P} \subseteq \iv{a, b}$.
% We would express this as 
% \begin{align}
%     \setop{sup} (\pzki{P}) &\leq b \\
%     \setop{inf} (\pzki{P}) & \geq a.
% \end{align}

\subsection{Trajectory Optimization}
\label{subsec:implementation_online}

Taking each of these constraints together, we can present an implementable version of the optimization program found in Section \ref{sec:algorithm_theory:optimization}:
\begin{align}
    \label{eq:pz_imp_optcost}
    &\underset{k \in K}{\min} &&\numop{cost}(k) \\
    \label{eq:pz_imp_opt}
    &&& h_{q^-}(i, j, k) \leq 0, \qquad &\forall i \in N_t, j \in N_q \\
    \label{eq:pz_imp_optpos_plus}
    &&& h_{q^+}(i, j, k) \leq 0 \qquad &\forall i \in N_t, j \in N_q \\
    \label{eq:pz_imp_optvel_minus}
    &&& h_{\dot{q}^-}(i, j, k) \leq 0 \qquad &\forall i \in N_t, j \in N_q \\
    \label{eq:pz_imp_optvel_plus}
    &&& h_{\dot{q}^+}(i, j, k) \leq 0 \qquad &\forall i \in N_t, j \in N_q \\
    \label{eq:pz_imp_opttorque_minus}
    &&& h_{u^-}(i, j, k) \leq 0 \qquad &\forall i \in N_t, j \in N_q \\
    \label{eq:pz_imp_opttorque_plus}
    &&& h_{u^+}(i, j, k) \leq 0 \qquad &\forall i \in N_t, j \in N_q \\
    % \label{eq:pz_imp_optposcon}
    % &&& \pzki{p_j} \subseteq [p_j^-, p_j^+] \qquad &\forall i, j \\
    % \label{eq:pz_optorncon1}
    % &&& \pzi{\hat{z}_{j}; k} \odot \pzi{\hat{z}_{d,j}}  \geq z_{d, j}^- \qquad &\forall i, j \\
    % \label{eq:pz_optorncon2}
    % &&& \pzk{\hat{x}_{j}} \odot \pz{\hat{x}_{d,j}}  \geq x_{d, j}^- \qquad &\forall i, j \\
    \label{eq:pz_imp_optcolcon}
    &&& \hobs(i, j, k, O) < 0 \qquad &\forall i \in N_t, j \in N_q, O \in \obsset.
\end{align}
The solver and hyperparameters used to solve this nonlinear program are detailed in Section \ref{sec:experiments:alg_implementation}.
Note that each of these constraints can be represented for each time interval $i$ in $\Nt$ in parallel. 
By applying Lemma \ref{lem:pz_opt_safe} one can prove that any feasible solution to this optimization problem can be tracked while satisfying joint limits, input limits, and without colliding into any obstacles. 

\input{algorithms/opt.tex}
\methodname's planning algorithm is summarized in Algorithm \ref{alg:opt}.
Note in particular, that the construction and solving of the optimization problem described in lines \eqref{eq:pz_imp_optcost}  -- \eqref{eq:pz_imp_optcolcon} is given $t\plan$ time. 
If a solution is not found within that time, then the output of Algorithm \ref{alg:opt} is set to $\texttt{NaN}$.

To facilitate real-time motion planning, we take steps to ensure that we can solve the optimization problem as quickly as possible. 
We therefore include the analytical constraint gradients when numerically solving the optimization problem.
As described above, each constraint contains a polynomial zonotope whose coefficients correspond to the trajectory parameters and are also the decision variables of the optimization problem.
Because each polynomial zonotope can be viewed as a polynomial function solely of the trajectory parameters, we can compute each constraint gradient with respect to the trajectory parameter $k$ using the standard rules of differential calculus, \emph{i.e.}, the power, product, and chain rules.

\subsection{\methodname{}'s Online Operation}

\input{algorithms/armourPlan.tex}

Algorithm \ref{alg:armourPlan} summarizes the online operation of \methodname{}. 
In particular, \methodname{} uses the robust passivity-based controller \eqref{eq:controller} to track the trajectory parameter computed at the previous planning iteration on Line \ref{lin:apply}. 
While this input is being applied, \methodname{} computes the trajectory to be tracked at the next planning iteration on Line \ref{lin:opt}.
Finally, by applying Corollary \ref{cor:tracking_error} and Lemma \ref{lem:pz_opt_safe}, one can prove that \methodname{} generates dynamically feasible, collision free behavior:
\begin{lem}[\methodname{} is Safe]
If $\qstart$ is collision free and one applies \methodname{}, as described in Algorithm \ref{alg:armourPlan}, then the robot is collision free. 
\end{lem}

We conclude by making a remark about applying \methodname{} to real-world systems. 
In practice, the robust passivity-based controller on Line \ref{lin:apply} is computed at discrete time instances at the input sampling rate requested by the robot.
As we describe in Section \ref{sec:experiments}, the input sampling rate of manipulator robots are typically a kilohertz or more \cite{kinova-user-guide,panda-user-guide}. 
Fortunately, the robust passivity-based controller can be computed at that rate. 
However, the input applied into the robot is usually zero-order held between sampling instances. 
To apply Corollary \ref{cor:tracking_error} in this instance, one would need to show that the tracking error bound was still satisfied if the input was applied in this zero-order held fashion.
Note, one could extend the results in this paper to address this additional requirement by extending the controller presented in this paper to deal with arbitrary bounded input disturbances \cite[(1)]{giusti2016bound}. 
However, this extension falls out of the scope of this paper. 


%~~~~~~~~~~~~~~~~~OVERFLOW
% We compose the offline reachable sets $\Zit$

% \thought{
% \begin{itemize}
%     \item \methodname computes trajectories online using the offline pz joint reachable sets
%     \item each pz jrs was computed assuming the initial position was 0 and some initial velocity
%     \item we create a rotation matrix from the initial position and rotate each pz jrs
%     \item since each pz jrs corresponds to a range of initial velocities we then slice the initial velocity
%     \item mention the offline reachable sets correspond to a set of desired trajectories. but since the robot is uncertain these trajectories aren't guaranteed to match the behavior of the robot
%     \item recall from section that the performance of the tracking controller was characterized by the ultimate bound
%     \item if we start within the ultimate bound, then we stay there for all time
%     \item ALSO MENTION THAT WE CREATE AN ERROR ZONOTOPE FOR THE ULTIMATE BOUND, SO IT REPRESENTS THE MAX DEVIATION FROM THE DESIRED TRAJECTORY
%     \item thus we can buffer the desired trajectory by adding the ultimate bound to get the actual JRS for the uncertain robot
%     \item we have an error pz for both position and velocity
%     \item The algorithm should \input{algorithms/createTraj}
%     \item \pat{At each time step, plug in intervals of t to get PZ overapproximation $\pz{\qdes}$ of $\qdes$... then add ultimate bound to get overapproximation $\pz{\q}$ of $\q$.}
%     \item \pat{can also describe sines/cosines for rotation matrices: $\pz{\cos{\qdes}}$, $\pz{\sin{\qdes}}$, etc.}
%     \item U-ARMTD begins by representing all possible parameterized trajectories of the robot starting from the initial condition $(\initq, \initdq)$.
%     \item The positions, velocities, and accelerations of each joint angle are represented by the polynomial zonotopes $\pzqjt$, $\pzqdjt$, $\pzqddjt$ respectively for $j = 1... n_q$ and $t \in T$ 
%     \item These sets are output by Algorithm \ref{alg:create_traj}, utilizing the precomputed reachable sets.
% \end{itemize}
% }

==> sections/misc_differentiating_interval_product.tex <==
\clearpage
\section*{Differentiating an Interval Product}

Let $T \subset \R$ denote time, $C \subset \R^2$ denote a configuration space, and $K \subset \R^n$ denote a trajectory parameter space.
Consider the interval matrix function $H: C\times K \to \pow{\R^{2\times 2}}$ for which
\begin{align}
    H(q,k) = \begin{bmatrix}
        I_1(q,k) & I_2(q,k) \\
        I_3(q,k) & I_4(q,k) \\
    \end{bmatrix},
\end{align}
where
\begin{align}
    I_i(q,k) = [l_i(q,k),\ u_i(q,k)]
\end{align}
(i.e., each $I_i$ is an interval).
Suppose that each $l_i, u_i: C\times K \to \R$ is differentiable with respect to $q$ and $k$.
Also consider the interval-valued trajectory $Q(\cdot,k): T \to \pow{C}$ parameterized by $k$, denoted
\begin{align}
    Q(t,k) = [q_l(t,k), q_u(t,k)]
\end{align}
and suppose $q_l$ and $q_u$ are differentiable with respect to $k$.
Denote
\begin{align}
    q_l = [q_{l,1}, q_{l,2}]\trans
\end{align}
as the lower bound of the 2-D interval returned by $Q$, and similarly for $q_u$.
Finally, consider the interval-valued function $P: T\times C\times K \to \pow{\R^2}$ given by
\begin{align}
    P(t,q,k) = H(q,k)Q(t,k).
\end{align}
We are concerned with finding the (sub)gradient
\begin{align}
    \nabla_k P.
\end{align}

Dropping the arguments for notation's sake, consider the first term of the product $H\cdot q$:
\begin{align}\label{eq:interval_product}
    I_1 q_l + I_2 q_u.
\end{align}
We can expand the lower bound of the first term (i.e., interval) in \eqref{eq:interval_product}, but the notation quickly becomes very busy with many subscripts.
So, for the sake of generality, consider the intervals
\begin{subequations}
\begin{align}
    I(q,k) &= [a(q,k),\ b(q,k)]\quad\regtext{and}\\
    Q(t,k) &= [c(t,k),\ d(t,k)],
\end{align}
\end{subequations}
with $a,b,c,d$ all differentiable with respect to $k$.
Dropping the arguments for the sake of notation, we can write an interval product
\begin{subequations}
\begin{align}
    I\cdot Q &= [x,y]\\
        &= [\min\left(ab,ad,bc,bd\right),\ \max\left(ac,ad,bc,bd\right)],\label{eq:interval_product_min_max}
\end{align}
\end{subequations}
where the lower/upper bounds $x,y: T\times C\times K \to \R$ are subdifferentiable with respect to $k$.
That is, we can find
\begin{align}
    \nabla_k x(t,q,k) = \nabla_k\left\langle ac\ \regtext{or}\ ad\ \regtext{or}\ bc\ \regtext{or}\ bd\right\rangle(t,q,k),\label{eq:interval_lower_bound_subgrad}
\end{align}
where $\langle{\cdot}\rangle$ are Shreyas' made-up notation to explain that we are taking $\nabla_k$ of whichever term in \eqref{eq:interval_product_min_max} achieves the min value to define $x$.
We can similarly find $\nabla_k y$.
Using interval addition, we can find $\nabla_k$ for the upper and lower bounds of the interval defined in \eqref{eq:interval_lower_bound_subgrad}.

==> sections/symbols.tex <==
\subsection{List of Symbols}
\begin{itemize}
%   \item $\int$:
%   \item $\pzg$
%   \item $\pzv$
%   \item $\pze$
%   \item $\pzn$
%   \item $\pzgi$
%   \item $\pzei$
%   \item $\interval{2}$:
%   \item $\pz{\dot{q}}$
%   \item $a_i$: DH parameter (link length?)
  \item $a_i^i$: acceleration of frame in expressed in frame i
  \item $a_{c,i}^i$: acceleration of link i com wrt frame i
  \item $a_0$: coefficient (but really center)
  \item $\pzei$: poly zonotope exponents
  \item $\robgain$: robust input "gain"
%   \item $\alpha_i$: link twist in DH convention
  \item $\beta_i$: zonotope indeterminants
  \item $c$: zonotope center
%   \item $c$: shorthand for cosine
%   \item $c_i^i$: 
  \item $c_{x_j}$: x-coordinate of COM of j-th link (same for y and z)
  \item $C$: Matrix zonotope center
  \item $C(q, \Delta)$: Coriolis matrix
%   \item $d_i$: DH parameter
  \item $\Delta$: vector of inertial parameters
  \item $\Delta_0$: vector of nominal inertial parameters
  \item $[\Delta]$: vector of interval inertial parameters
  \item $\pz{\Delta}$: vector of PZ inertial parameters
  \item $e$: vector of joint position errors
  \item $\dot{e}$: vector of joint velocity errors
  \item $\pbound$: ultimate position bound for single joint
  \item $\vbound$: ultiamte velocity bound for single joint
  \item $\pboundvec$: vector of ultimate position bounds
  \item $\vboundvec$: vector of ultimate velocity bounds
  \item $f_i^i$: Force at joint
  \item $F_i^i$: Force at center of mass
  \item $\FK_i(q)$: forward kinematics
  \item $\FO_i(q)$: forward occupancy
  \item $\robcoeff$: robust input coefficient
  \item $g_i$: ith zonotope generator
  \item $\pzgi$: ith PZ coefficient (aka generator)
  \item $G_i$:  ith generator matrix of Matrix zonotope 
  \item $G(q, \Delta)$: gravity vector
  \item $\kscale$: scale for $k$ interval
  \item $\robh$: control barrier function
  \item $\robH$: forward invariant set associated with $\robh$
  \item $i$: time index
  \item $I_i^i$: link i inertia tensor wrt frame i
  \item $j$: joint index
%   \item $\mathcal{J}_i$: joint reachable set
%   \item $J_i(t)$: offline overapproximation of joint reachable set
  \item $k$: trajectory parameter
  \item $K$: space of trajectory parameters
  \item $K_r$: gain matrix
  \item $\kappa_P$: robust controller gain
  \item $L_i$: volume of link i
%   \item $\lambda_j$: indeterminants
  \item $\lambda_{min}$: smallest eigenvalue
  \item $\lambda_{max}$: largest eigenvalue
  \item $m_i$: mass of link i
  \item $M$: matrix zonotope
%   \item$\Mit$: matrix zonotope as a function of time
  \item $M$: Mass matrix
  \item $\pz{M}$: poly zonotope Mass matrix
  \item $\pz{M(\pz{\q})}$: pz mass matriz as a function of pz state.
  \item $M(\q, \Delta)$ true mass matrix at $\q$
  \item $n$: generic constant
  \item $\nq$: number of joints
  \item $\nt$ number of time steps
%   \item $n_{n_q}^{n_q}$: moment
  \item $\nObs$: number of obstacles
  \item $N_i^i$: moment
  \item $O_j$: Obstacle $j$ where $j$ is a generic index
%   \item $\mathcal{O}$: set of all obstacles
  \item $\obsset$: set of all obstacles
  \item $\mathbb{N}$: natural numbers
  \item $\pzn$: number of PZ generators
  \item $p_1$: generic point inside poly zonotope
  \item $p_2$: generic point inside poly zonotope
  \item $p_i$: position of frame $i$ relative to frame $0$
  \item $p_{i-1,i}^i$: position of frame i wrt frame i-1 expressed in frame i \jon{i think this is not needed}
%   \item $PZ$: generic polynomial zonotope
  \item $\pz{P_1}$: generic polynomial zonotope
  \item $\pz{P_2}$: generic polynomial zonotope
%   \item $\mathcal{ABCPZ}$: Polynomial Zonotope
%   \item $[\Phi]$: interval disturbance
%   \item $\varphi_P$: robust controller gain
  \item $q$: vector of joint positions
  \item $\qd$: vector of joint velocities
  \item $\qdd$: vector of joint accelerations
  \item $\initq$: estimate of initial position
  \item $\initdq$: estimate of initial velocity
  \item $\qdes$: desired joint positions
  \item $\qdesdot$: desired joint velocities
  \item $\qdesddot$: desired joint accelerations
  \item $\qadot$: modified velocity trajectory
  \item $\qaddot$: modified acceleration trajectory
  \item $\pzqji$: poly zonotope representation of $q$ at $i$\ts{th} time step
  \item $\pzqdji$: poly zonotope representation of $\qd$ at $i$\ts{th} time step
  \item $Q$: configuration space
  \item $\robr$: modified error
  \item $R_{i-1}^i$: orientation of frame $i-1$ \textit{wrt} frame $i$
%   \item $^{i}R_{i-1}$: orientation of frame $i-1$ \textit{wrt} frame $i$
  \item $R_i(q)$: orientation of frame $i$ \textit{wrt} frame $0$
  \item $\pz{R_{i-1}^i}$: poly zonotope representation of orientation of frame $i-1$ \textit{wrt} frame i
  \item $\mathbb{R}^n$: reals 
%   \item $\rho$: worst-case disturbance
%   \item $s$: shorthand for sine
%   \item $S_i(t)$: sliced reachable set
  \item $\sigma$: coefficient to be sliced/evaluated
  \item $\sigma_m$: uniform bound
  \item $\sigma_M$: uniform bound
  \item $t$: time
  \item $T$: time interval
  \item $\tau$: nominal control input
  \item $u$: control input
%   \item $U_i(t)$: overapproximation of input reachable set
  \item $\robv$: robust control input
  \item $\roblyap$: Lyapunov function
  \item $\roblevel$: Lyapunov function threshold
%   \item $V_i(t)$: zonotope representation of link i volume
  \item $w$: disturbance due to inertial uncertainty
  \item $\normwmax$ norm of max disturbance
  \item $W$: workspace
  \item $\omega_i^i$: frame i angular velocity wrt frame i
  \item $\dot{\omega}_i^i$: frame i angular acceleration wrt frame i
  \item $\pzv$: indeterminant for polynomial zonotope
%   \item $x$: generic interval
%   \item $y$: generic interval
%   \item $z$: generic point inside zonotope
  \item $z_i$: frame i axis of rotation (expressed in base frame?)
  \item $Z$: generic zonotope
  \item $Z_1$: generic zonotope
  \item $Z_2$: generic zonotope
\end{itemize}
